SyGuS Techniques in the Core of an SMT Solver

We give an overview of recent techniques for implementing syntax-guided synthesis (SyGuS) algorithms in the core of Satisfiability Modulo Theories (SMT) solvers. We define several classes of synthesis conjectures and corresponding techniques that can be used when dealing with each class of conjecture.

==> eptcsdata.tex <==
\providecommand{\firstpage}{81}
\providecommand{\publicationstatus}{D. Fisman, S. Jacobs (Eds.): Sixth Workshop on Synthesis (SYNT 2017)\\
EPTCS 260, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.260.8}{10.4204/EPTCS.260.8}}

